3DSS: 3D Surface Splatting for Inverse Rendering

We present 3D Surface Splatting (3DSS), the first differentiable surface splatting renderer for physically-based inverse rendering from multi-view images. Our central insight is that surface separation, which groups the surfels covering a pixel by the surface they sample, can be formulated with the reconstruction kernels themselves: two surfels sample the same surface when their kernels overlap in depth. Compositing each resulting surface layer with a coverage opacity derived from its accumulated Elliptical Weighted Average (EWA) weight yields anti-aliased silhouettes and informative visibility gradients at sparsely covered edges. With forward microfacet shading under co-optimized HDR environment lighting, 3DSS jointly recovers shape, spatially-varying BRDF, and illumination, and its oriented surfels convert directly into meshes by oriented-point surface reconstruction. On the real-world Stanford-ORB and the TensoIR Synthetic benchmarks, 3DSS outperforms state-of-the-art mesh-based and major comparable implicit and Gaussian-based methods in novel view synthesis and relighting, with geometry on par with the strongest baselines.

==> preamble.tex <==

\makeatletter
\@ifpackageloaded{lineno}{%
  \@ifpackagelater{lineno}{2026/02/11}{%
    \IfFormatAtLeastTF{2025-06-01}{%
      \RemoveFromHook{build/column/before}[lineno]%
      \AddToHook{build/column/after}[lineno-columnfix]{%
        \setbox\@outputbox\vbox{%
          \boxmaxdepth\@maxdepth
          \protected@write\@auxout{}{%
            \string\def\string\@LN@column{\if@firstcolumn1\else2\fi}}%
          \box\@outputbox}}%
    }{}%
  }{}%
}{}
\makeatother

\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{\textbf{\textcolor{red}{TODO: #1}}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}

\usepackage{microtype}

\makeatletter
\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}{.5em \@plus .25em \@minus .1em}{-1em}{\normalfont\normalsize\bfseries}}
\makeatother

\setlength{\abovecaptionskip}{.5em}

\usepackage{multirow}
\usepackage{colortbl}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{float}
\usepackage{wrapfig}
\usepackage{mathtools}

\newcommand{\CropParams}{trim={80 80 80 80},clip}       %
\newcommand{\CompColWidth}{0.099\textwidth}              %
\newcommand{\figimg}{\includegraphics}

\newcommand{\first}[1]{\cellcolor[HTML]{F1948A}#1}
\newcommand{\second}[1]{\cellcolor[HTML]{F8C471}#1}
\newcommand{\third}[1]{\cellcolor[HTML]{F9E79F}#1}

\everydisplay\expandafter{%
  \the\everydisplay
  \abovedisplayskip=4pt plus 2pt minus 2pt
  \belowdisplayskip=4pt plus 2pt minus 2pt
  \abovedisplayshortskip=2pt plus 1pt minus 1pt
  \belowdisplayshortskip=2pt plus 1pt minus 1pt
}
\setlength{\textfloatsep}{10pt plus 2pt minus 2pt}

\makeatletter
\@ifundefined{Gread@transgrouptrue}{}{\let\Gread@transgrouptrue\Gread@transgroupfalse}
\makeatother

